What are the Machine Learning best practices reported by practitioners on Stack Exchange?

Machine Learning (ML) is being used in multiple disciplines due to its powerful capability to infer relationships within data. In particular, Software Engineering (SE) is one of those disciplines in which ML has been used for multiple tasks, like software categorization, bugs prediction, and testing. In addition to the multiple ML applications, some studies have been conducted to detect and understand possible pitfalls and issues when using ML. However, to the best of our knowledge, only a few studies have focused on presenting ML best practices or guidelines for the application of ML in different domains. In addition, the practices and literature presented in previous literature (i) are domain-specific (e.g., concrete practices in biomechanics), (ii) describe few practices, or (iii) the practices lack rigorous validation and are presented in gray literature. In this paper, we present a study listing 127 ML best practices systematically mining 242 posts of 14 different Stack Exchange (STE) websites and validated by four independent ML experts. The list of practices is presented in a set of categories related to different stages of the implementation process of an ML-enabled system; for each practice, we include explanations and examples. In all the practices, the provided examples focus on SE tasks. We expect this list of practices could help practitioners to understand better the practices and use ML in a more informed way, in particular newcomers to this new area that sits at the intersection of software engineering and machine learning.

==> table_practices_dcl.tex <==


\begin{small}
	\setlength{\tabcolsep}{3pt}
   \begin{longtable}{M{20pt} m{320pt}}
		
		\caption{Validated practices in Data Cleaning} \label{tab:pr_dcl} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{2}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{2}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		\hline
		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Data  Cleaning (dcl)}}\\
	%	\midrule
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} \\
		\midrule
		\multicolumn{2}{c}{\emph{Exploratory Data Analysis (EDA)}}\\
		\midrule[0.03em]
		\textbf{\acron[M]{dcl}{1}} & For each possible attribute/column in a dataset, we should identify its type before applying any pre-processing technique \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{2}} & It should be determined what variables are dependent and what ones are independent. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{3}} &When analyzing time series/temporal data, possible temporal trends should be identified. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{4}} & When analyzing time series/temporal data, weird trends should be identified. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{5}}  &It is needed to identify missing values and their nature before doing any pre-processing. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{6}} & Before applying any pre-processing technique, potential errors in data should be identified. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{7}} & If correlation between existing features and instances of geographical data are needed, then, geographical data should be clustered \\  \addlinespace[1pt] 
		
		\midrule
		\multicolumn{2}{c}{\emph{Data}}\\
		\midrule
		\textbf{\acron[M]{dcl}{8}} & For improving model performance with a dataset that has a categorical feature, the data should be split by each category. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{9}} & If it is needed to optimize hyper-parameters, the dataset should be split into training, validation and test sets in order to prevent overfitting and avoid biased computing metrics \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{10}} & In order to prevent overfitting and avoid biased metrics when optimizing, the whole dataset should be divided into train and test; then, the training data should be divided into folds for cross-validation.\\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{11}} & The size of a dataset should be only calcuated after the data pre-processing. \\  \addlinespace[1pt] 
		
		\midrule
		\multicolumn{2}{c}{\emph{Wrangling}}\\ 
		\midrule
		\textbf{\acron[M]{dcl}{12}}  & If an imputation technique is used, the same technique should be used in the training, validation and testing sets.  \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{13}} & When having an unbalanced dataset, balancing the data should be done only in the training dataset. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{14}} & When undersampling data, the samples that are being selected should be randomly sampled. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{15}}  &Oversampling should be done only after the whole dataset is split into train, validation and test sets. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{16}} & Transformation of numerical data should be done in all the sets by using the statistics computed on the training data.\\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{17}} &Transformations should take into account (i) the model that is going to be used and (ii) the data nature. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{18}} &Features/attributes should be scaled when using a SVM model. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{19}}& When transforming numerical data into ratios and the transformation leads to infinite values, smoothing should be used. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{20}}& if an algorithm does not support categorical data, this type of feature should be encoded into multiple binary features or by counting frequencies. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{21}} & Datetime data could be partitioned into their corresponding components. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{22}} & Data augmentation should be used in order to prevent overfitting. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{23}}  & For analyzing handwritten text images, the image should be split into individual characters. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{24}} & If the task of a model is detect objects, then, each ROI should be cropped instead of using the complete image. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{25}} & When handling geographical data and the latitude and longitude will be transformed, directional statistics  should be used to deal with potential interdependence of latitude and longitude, and with scales wrapping around\\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{26}} & When handling geographical data, the geodesic distance should be used to compute the distance between two points of interest. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{27}} & If a variable is dependable on time along with other features, then, the timeseries variable could be encoded as frequencies. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{28}} & When encoding geographical data, Sine and Cosine facets could be used for representing the cyclical characteristics from date time features. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{29}} &  If noise in data is present in a dataset, then, it should be removed, with techniques such as smoothing. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{30}} & If ReLU is being used as an activation function in Neural Networks (NN), then, the features should be scaled. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{31}} & If clustering is needed and the dataset contains aggregated structures, and the order of the aggregated data matters, then, a new feature should be created in to encode the order. \\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{32}} & When working with an LSTM network the sequences that are going to be fed into the NN should be padded in order to equalize the length of all the sequences.\\ \cmidrule[0.01em]{1-2} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{33}} & When data is being anonymized with hashing, it should be done over a unique identifier using salt. \\ \addlinespace[1pt] 
		\bottomrule
	\end{longtable}
\end{small}


==> table_practices_dcl2.tex <==
\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Data Cleaning - EDA subcategory. Including the extra considerations, where   P - Phase category related  notes, C - additional clarifications} \label{tab:pr_dcl_eda} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		
		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Data  Cleaning (dcl)}}\\
		%	\midrule
		\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
				\textbf{Validated*}  \end{tabular}
		}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
			\textbf{Extra**} \end{tabular} }\ \\
		\midrule
		%\multicolumn{2}{c}{\emph{Exploratory Data Analysis (EDA)}}\\
		%\midrule[0.03em]
		\textbf{\acron[M]{dcl}{1}} & For each possible attribute/column in a dataset, we should identify its type before applying any pre-processing technique &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{2}} & It should be determined what variables are dependent and what ones are independent. &4&C\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{3}} &When analyzing time series/temporal data, possible temporal trends should be identified. &4 &-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{4}} & When analyzing time series/temporal data, weird trends should be identified.  &4&- \\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{5}}  &It is needed to identify missing values and their nature before doing any pre-processing. &4 &-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{6}} & Before applying any pre-processing technique, potential errors in data should be identified. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{7}} & If correlation between existing features and instances of geographical data are needed, then, geographical data should be clustered. &3&-\\  \addlinespace[1pt] 
	
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\vspace{-7pt}
\end{small}

==> table_practices_dcl3.tex <==
\begin{small}
	\setlength{\tabcolsep}{2.5pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Data Cleaning  - Data subcategory. Including the extra considerations,  P - Phase category related  notes, C - additional clarifications} \label{tab:pr_dcl_data} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline
		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Data  Cleaning (dcl)}}\\
		%	\midrule
		\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
				\textbf{Validated*}  \end{tabular}
		} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
			\textbf{Extra**}  \end{tabular} }\\
		\midrule
		\textbf{\acron[M]{dcl}{8}} & For improving model performance with a dataset that has a categorical feature, the data should be split by each category. &4&P\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{9}} & If it is needed to optimize hyper-parameters, the dataset should be split into training, validation and test sets in order to prevent overfitting and avoid biased computing metrics. &4 &P\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{10}} & In order to prevent overfitting and avoid biased metrics when optimizing, the whole dataset should be divided into train and test; then, the training data should be divided into folds for cross-validation.&3&P\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dcl}{11}} & The size of a dataset should be only calcuated after the data pre-processing. &3&-\\  \addlinespace[1pt] 
		
		\bottomrule 
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}

\end{small}

==> table_practices_dcl4.tex <==
\begin{small}
	\setlength{\tabcolsep}{3pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for  Data Cleaning - Wrangling subcategory. Including the extra considerations, where  P - Phase category related  notes, C - additional clarifications}
		\vspace{-0.3cm}
		 \label{tab:pr_dcl_wrangling} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline
		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Data  Cleaning (dcl)}}\\
		%	\midrule
		\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
				\textbf{Validated*}  \end{tabular}
		} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
			\textbf{Extra**}  \end{tabular} }\\
		\midrule
		\textbf{\acron[M]{dcl}{12}}  & If an imputation technique is used, the same technique should be used in the training, validation and testing sets. & 4&C \\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{13}} & When having an unbalanced dataset, balancing the data should be done only in the training dataset. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{14}}  &Oversampling should be done only after the whole dataset is split into train, validation and test sets. & 4&P\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{15}} & When undersampling data, the samples that are being selected should be randomly sampled. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{16}} & Transformation of numerical data should be done in all the sets by using the statistics computed on the training data. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{17}} &Transformations should take into account (i) the model that is going to be used and (ii) the data nature. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{18}} &Features/attributes should be scaled when using a SVM model. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{19}}& When transforming numerical data into ratios and the transformation leads to infinite values, smoothing should be used. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{20}}& if an algorithm does not support categorical data, this type of feature should be encoded into multiple binary features or by counting frequencies. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{21}} & Datetime data could be partitioned into their corresponding components. & 4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{22}} & Data augmentation should be used in order to prevent overfitting. & 4&C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{23}}  & For analyzing handwritten text images, the image should be split into individual characters. & 4 &C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{24}} & If the task of a model is detecting objects, then, each ROI should be cropped instead of using the complete image. & 3&C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{25}} & When handling geographical data and the latitude and longitude will be transformed, directional statistics  should be used to deal with potential interdependence of latitude and longitude, and with scales wrapping around & 3&C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{26}} & When handling geographical data, the geodesic distance should be used to compute the distance between two points of interest. & 3 &C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{27}} & If a variable is dependable on time along with other features, then, the timeseries variable could be encoded as frequencies. & 3&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{28}} & When encoding geographical data, Sine and Cosine facets could be used for representing the cyclical characteristics from date time features. & 3&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{29}} &  If noise is present in a dataset, then, it should be removed, with techniques such as smoothing. & 3 &P\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{30}} & If ReLU is being used as an activation function in Neural Networks (NN), then, the features should be scaled. & 3&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{31}} & If clustering is needed and the dataset contains aggregated structures, and the order of the aggregated data matters, then a new feature should be created in to encode the order. & 3&-\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{32}} & When working with an LSTM network the sequences that are going to be fed into the NN should be padded in order to equalize the length of all the sequences. & 3&C\\ \cmidrule[0.01em]{1-4} \addlinespace[0.5pt] 
		\textbf{\acron[M]{dcl}{33}} & When data is being anonymized with hashing, it should be done over a unique identifier using salt. & 3&P\\ \addlinespace[0.5pt] 
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\end{small}

==> table_practices_dl.tex <==


\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 

		
		\caption{Validated practices for Data Labeling. Including the extra considerations, where P - Phase category related  notes, C - additional clarifications} \label{tab:pr_dl} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline
		\endlastfoot
	%	\multicolumn{1}{c}{\textbf{Data  Labeling (dl)}}\\
		%\midrule
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*}  \end{tabular}
	 	}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**}  \end{tabular} }\\
		\midrule
		\textbf{\acron[M]{dl}{1}} & Manual data labeling could be expensive, so it could be done by more than one person in order to scale the labeling process. & 4&- \\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\textbf{\acron[M]{dl}{2}}  & In the case of object detection, when selecting the region of interest, a tool should be used to fix the aspect ratio for all the labeled objects. & 3 &- \\ \addlinespace[1pt] 
		
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{4}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{4}{l}{** Extra considerations}

	\end{longtable}
\end{small}


==> table_practices_fe.tex <==


\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Feature Engineering. Including the extra considerations, where P - Phase category related  notes,  C - additional clarifications} \label{tab:pr_fe} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline 
		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Feature Engineering (fe)}}\\
		%\midrule
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*}  \end{tabular}
	 	} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**}  \end{tabular} }\\
		\midrule
		\acron[M]{fe}{1} & Feature engineering should be only executed with the training data and without taking into account the whole dataset.&4 &-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{2} &Multivariate feature engineering is preferred over univariate feature selection. &4&C\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{3} &It is relevant to check existing techniques of dimensionality reduction. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{4} &When using feature selection algorithms, it is important to evaluate which are their assumptions and if they hold for a particular case. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{5} &When using the  PCA method, its assumptions should be checked.&3 &C \\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{6} &When selecting features, the existing techniques for this purpose should be checked. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{7} &When using Logistic Regression for selecting features, select the significant ones. &3&C\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{8} &Regardless the classifier that is being used,  mutual information techniques for feature selection should be considered. &3&C\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{9} &Using backward and forward feature selection should be taken into account regardless the classifier that is being used. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{10} &For feature selection, the regularization techniques that are part of the algorithm should be considered (e.g., Lasso, Elastic Net when high collinearity). &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{fe}{11}  &The usage of Lasso, Ridge, or Glmnet or feature selection in a multiple regression model should be considered. &3&-\\
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\vspace{-8.2pt}
\end{small}


==> table_practices_general.tex <==


\begin{small}
	\begin{longtable}{p{340pt}}
		
		\caption{Discussed and validated best \ac{ML} practices in \ac{STE} communities} \label{tab:BP_rq1} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{1}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{1}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		\hline \hline
		\endlastfoot
		\multicolumn{1}{c}{\textbf{Model Requirement (mr)}}\\
		\midrule
		%\the\textwidth\\
		\textbf{\acron[M]{mr}{1}}  The goal of the model that is going to be trained should be considered when selecting the most appropriate metrics for assessing the model performance. \\
		\textbf{\acron[M]{mr}{2}}  It is important to identify the needs/requirements of model retraining.\\
		\textbf{\acron[M]{mr}{3}} If a ML model is published as a cloud service, specifically, when  a classification/prediction task uses ML cloud-based services, it is important  to define the use case and the model requirements in order to identify how frequently the service should be invoked. \\
		\textbf{\acron[M]{mr}{4}} When using probabilistic forecasting in a decision system, it is necessary to decouple the probabilistic model optimization from the probability threshold selection. \\
		
		
		\midrule
		\multicolumn{1}{c}{\textbf{Data Collection (dc)}}\\
		\midrule
		\textbf{\acron[M]{dc}{1}}  The distribution of the training data should reflect the real distribution. \\
		\textbf{\acron[M]{dc}{2}}  If a model is expected to detect ''something" in an image, then representative examples of that ``something" should be present in the training and testing data.\\
		\textbf{\acron[M]{dc}{3}} When measuring a dataset size it should not be done only by referring to storage space but also in terms of rows and columns. \\
		\textbf{\acron[M]{dc}{4}} If it is required to augment the number of instances in the negative class, preexisting datasets could be used for including more instances in the dataset.\\
		\textbf{\acron[M]{dc}{5}} The images that are going to be used as instances of the negative class should have some common characteristics with the positive ones.\\
		\textbf{\acron[M]{dc}{6}} The minimum size of the object that is going to be detected should be present in the data that is going to be used for training the model.\\
		\textbf{\acron[M]{dc}{7}} The object ROI should have a similar aspect ratio in all the positive images. \\
		
		\midrule
		\multicolumn{1}{c}{\textbf{Data  Cleaning (dcl)}}\\
		\midrule
		\textbf{\acron[M]{dcl}{1}}  For each possible attribute/column in a dataset, we should identify its type before applying any pre-processing technique \\
		\textbf{\acron[M]{dcl}{2}}  It should be determined what variables are dependent and what ones are independent. \\
		\textbf{\acron[M]{dcl}{3}} When analyzing time series/temporal data, possible temporal trends should be identified. \\
		\textbf{\acron[M]{dcl}{4}}  When analyzing time series/temporal data, weird trends should be identified. \\
		\textbf{\acron[M]{dcl}{5}}  It is needed to identify missing values and their nature before doing any pre-processing. \\
		\textbf{\acron[M]{dcl}{6}}  Before applying any pre-processing technique, potential errors in data should be identified. \\
		\textbf{\acron[M]{dcl}{7}}  If correlation between existing features and instances of geographical data are needed, then, geographical data should be clustered \\
		\textbf{\acron[M]{dcl}{8}}  For improving model performance with a dataset that has a categorical feature, the data should be split by each category. \\
		\textbf{\acron[M]{dcl}{9}}  If it is needed to optimize hyper-parameters, the dataset should be split into training, validation and test sets in order to prevent overfitting and avoid biased computing metrics \\
		\textbf{\acron[M]{dcl}{10}} In order to prevent overfitting and avoid biased metrics when optimizing, the whole dataset should be divided into train and test; then, the training data should be divided into folds for cross-validation.\\
		\textbf{\acron[M]{dcl}{11}}  The size of a dataset should be only calcuated after the data pre-processing. \\
		\textbf{\acron[M]{dcl}{12}}  If an imputation technique is used, the same technique should be used in the training, validation and testing sets.  \\
		\textbf{\acron[M]{dcl}{13}}  When having an unbalanced dataset, balancing the data should be done only in the training dataset. \\
		\textbf{\acron[M]{dcl}{14}}  When undersampling data, the samples that are being selected should be randomly sampled. \\
		\textbf{\acron[M]{dcl}{15}}  Oversampling should be done only after the whole dataset is split into train, validation and test sets. \\
		\textbf{\acron[M]{dcl}{16}}  Transformation of numerical data should be done in all the sets by using the statistics computed on the training data.\\
		\textbf{\acron[M]{dcl}{17}} Transformations should take into account (i) the model that is going to be used and (ii) the data nature. \\
		\textbf{\acron[M]{dcl}{18}} Features/attributes should be scaled when using a SVM model. \\
		\textbf{\acron[M]{dcl}{19}} When transforming numerical data into ratios and the transformation leads to infinite values, smoothing should be used. \\
		\textbf{\acron[M]{dcl}{20}} if an algorithm does not support categorical data, this type of feature should be encoded into multiple binary features or by counting frequencies. \\
		\textbf{\acron[M]{dcl}{21}}  Datetime data could be partitioned into their corresponding components. \\
		\textbf{\acron[M]{dcl}{22}}  Data augmentation should be used in order to prevent overfitting. \\
		\textbf{\acron[M]{dcl}{23}}  For analyzing handwritten text images, the image should be split into individual characters. \\
		\textbf{\acron[M]{dcl}{24}}  If the task of a model is detect objects, then, each ROI should be cropped instead of using the complete image. \\
		\textbf{\acron[M]{dcl}{25}} When handling geographical data and the latitude and longitude will be transformed, directional statistics  should be used to deal with potential interdependence of latitude and longitude, and with
		scales wrapping around\\
		\textbf{\acron[M]{dcl}{26}} When handling geographical data, the geodesic distance should be used to compute the distance between two points of interest. \\
		\textbf{\acron[M]{dcl}{27}}  If a variable is dependable on time along with other features, then, the timeseries variable could be encoded as frequencies. \\
		\textbf{\acron[M]{dcl}{28}}  When encoding geographical data, Sine and Cosine facets could be used for representing the cyclical characteristics from date time features. \\
		\textbf{\acron[M]{dcl}{29}}  If noise in data is present in a dataset, then, it should be removed, with techniques such as smoothing. \\
		\textbf{\acron[M]{dcl}{30}}  If ReLU is being used as an activation function in Neural Networks (NN), then, the features should be scaled. \\
		\textbf{\acron[M]{dcl}{31}}  If clustering is needed and the dataset contains aggregated structures, and the order of the aggregated data matters, then, a new feature should be created in to encode the order. \\
		\textbf{\acron[M]{dcl}{32}}  When working with an LSTM network the sequences that are going to be fed into the NN should be padded in order to equalize the length of all the sequences.\\
		\textbf{\acron[M]{dcl}{33}}  When data is being anonymized with hashing, it should be done over a unique identifier using salt. \\
		
		\midrule
		\multicolumn{1}{c}{\textbf{Data  Labeling (dl)}}\\
		\midrule
		\textbf{\acron[M]{dl}{1}}  Manual data labeling could be expensive, so it could be done by more than one person in order to scale the labeling process. \\
		\textbf{\acron[M]{dl}{2}}  In the case of object detection, when selecting the region of interest, a tool should be used to fix the aspect ratio for all the labeled objects.\\
		
		
		\midrule
		\multicolumn{1}{c}{\textbf{Feature Engineering (fe)}}\\
		\midrule
		\acron[M]{fe}{1} Feature engineering should be only applied to the training data and without taking into account the whole dataset. \\
		\acron[M]{fe}{2} Multivariate feature engineering is preferred over univariate feature selection \\
		\acron[M]{fe}{3} It is relevant to check existing techniques of dimensionality reduction.\\
		\acron[M]{fe}{4} When using feature selection algorithms it is important to evaluate which are their assumptions and if they hold for a particular case.\\
		\acron[M]{fe}{5} When using the  PCA method, its assumptions should be checked. \\
		\acron[M]{fe}{6} When selecting features, the existing techniques for this purpose should be checked. \\
		\acron[M]{fe}{7} When using Logistic Regression for selecting features, select the significant ones. \\
		\acron[M]{fe}{8} Regardless the classifier that is being used,  mutual information techniques for feature selection should be considered. \\
		\acron[M]{fe}{9} Using backward and forward feature selection should be taken into account regardless the classifier that is being used. \\
		\acron[M]{fe}{10} For feature selection, the regularization techniques that are part of the algorithm should be considered (e.g., Lasso, Elastic Net when high collinearity).\\
		\acron[M]{fe}{11} The usage of Lasso, Ridge, or Glmnet or feature selection in a multiple regression model should be considered.\\
		
		\\
		\midrule
		\multicolumn{1}{c}{\textbf{Model Training (mt)}}\\
		\midrule
		\acron[M]{mt}{1} If the objective is to build specialized models, then a specific model for each category in a categorical feature should be trained.\\
		\acron[M]{mt}{2} If the dataset that is going to be used has multiple features in different scale systems, then, invariant-algorithms like tree based algorithms should be used.\\
		\acron[M]{mt}{3} When training prediction models with time series data, then, sliding windows should be used.\\
		\acron[M]{mt}{4} Test data should not be included in the training data in order to have a fair metric\\		
		\acron[M]{mt}{5}  As many data as possible should be used when training a model\\		
		\acron[M]{mt}{6} When training a NN, drop out layer(s) should be used to avoid overfitting\\	
		\acron[M]{mt}{7} If symmetry is needed to be avoided, in a NN, their components should be initialized with different values.\\	
		\acron[M]{mt}{8} Neural Networks should be initialized randomly.\\	
		\acron[M]{mt}{9} When training a NN Early Stopping should be used.\\	
		\acron[M]{mt}{10} If images are being used for NN training, it is preferable a convolutional layer than a fully connected one.\\	
		\acron[M]{mt}{11} If a neural network stagnates with non optimal results, then the learning rate should be decreased.\\	
		\acron[M]{mt}{12} If there is not enough data when training a deep NN from scratch, transfer learning with fine tuning should be tried.\\	
		\acron[M]{mt}{13} If a deep NN does not converge in an specific number of iterations, then increasing this number should be tried.\\	
		\acron[M]{mt}{14} When having a large dataset that does not fit in memory, multiples models could be first trained on random data samples, and then an ensemble with those models could be created to get a more accurate model than a base learner with fewer data.\\	
		\acron[M]{mt}{15} A model should be retrained with an online approximation if the model needs to dynamically adapt to new patterns from the data.\\	
		\acron[M]{mt}{16} If dependencies between features exist, it is suggested to used GBDT instead of a Random Forest\\	
		\acron[M]{mt}{17} The number of parameters of a deep NN should be proportional to the number of instances needed for training a deep NN.\\	
		\acron[M]{mt}{18} If there is a large data variance, the number of layers in a NN must be increased.\\	
		\acron[M]{mt}{19} A NN should be trained with different initialized weights in several times, in order to first get an average of the results and its variance and then to get a more specific judgment of the overall performance.\\	
		\acron[M]{mt}{20} If a NN does not converge, then, the learning rate should be reduced by a half or one third\\	
		\acron[M]{mt}{21} When a NN does not converge, the size of the mini-batches should be increased.\\	
		\acron[M]{mt}{22} For faster convergence of Multi Layer Perceptrons SGD should be used.\\	
		\acron[M]{mt}{23} If robustness is required in a \ac{ML} model, then, Adversarial Machine learning should be used.\\	
		\acron[M]{mt}{24} If the time-performance of a model is being affected due to a large time series data, then the data could be sub-sampled.\\	
		\acron[M]{mt}{25} When sub-sampling time-series data, it should be checked that unwanted confounding between sampled origins and seasonality in data is not being introduced. \\	
		\acron[M]{mt}{26} Before combining models, the correlation of models' prediction should be measured\\	
		\acron[M]{mt}{27} Only independent models should be combined in an ensemble.\\	
		\acron[M]{mt}{28} When training a model with mixed type features, which includes time series features, separate models for each part of the representation should be built, and then the different models should be combined in an ensemble.\\	
		\acron[M]{mt}{29} When using clustering, the model should be re-trained with new data to build more clusters and increase its efficiency.\\	
		\acron[M]{mt}{30} In order to deal with concept drift when working with data streams, models should be retrained with small a limited number of instances.\\	
		\acron[M]{mt}{31} A model should be retrained in offline mode, due to this approximation could lead to a better global approximation.\\	
		\acron[M]{mt}{32} In the case of online and offline re-training are not an option, then using batch/mini-batch approach should be used.\\	
		\acron[M]{mt}{33} The optimization process should be done with a validation set\\	
		\acron[M]{mt}{34} Each model that is combined into an ensemble should be optimized independently.\\	
		\acron[M]{mt}{35} In order to monitor the learning process's evolution, the model's predefined metrics should be calculated at the end of each epoch.\\	
		\acron[M]{mt}{36} When data is insufficient to split it into train, validation and test, then cross-validation should be used\\	
		\acron[M]{mt}{37} It is preferable to use cross-validation instead of a training and test data split for training and testing a model.\\	
		\acron[M]{mt}{38} It is preferable to use nested cross-validation instead of a training and test split for training and testing a model\\	
		\acron[M]{mt}{39} When training NN in order to ensure reproducibility and fair comparison, the seed used for generating random numbers in the training process should be fixed.\\	
		\acron[M]{mt}{40} In order to prevent overfitting, cross-validation should be used.\\	
		\acron[M]{mt}{41} In order to avoid overfitting nested cross-validation should be used .\\
		\acron[M]{mt}{42} First tune the hyper-parameters of the  probabilistic model and then adjust the decision thresholds.\\
		\acron[M]{mt}{43} In order to monitor the evolution of the learning process and identify issues at an early stage on it, learning curves should be plotted.\\
		\acron[M]{mt}{44} When evaluating a model bootstrapping or cross-validation should be tried.\\
		\acron[M]{mt}{45} When training/validating/testing a model, the process of cross-validation should be repeated with different seeds to prevent the impact of using a fixed seed.\\
		\acron[M]{mt}{46} If you want to lower the uncertainty of the hyper-parameter tuning process, then nested cross-validation should be used.\\
		\acron[M]{mt}{47} In order to avoid overfitting the performance between training and testing should be compared.\\
		
		\\
		\midrule
		\multicolumn{1}{c}{\textbf{Model Evaluation (me)}}\\
		\midrule
		\acron[M]{me}{1} Use Adversarial inputs for testing a model in order to ensure robustness.\\
		\acron[M]{me}{2} After the best hyper-parameters are found, the model with those ``optimum" hyper-parameters should be tested in the set built for testing.\\
		\acron[M]{me}{3} If a superset vocabulary was built for a NLP task, then the model bias should be checked.\\
		\acron[M]{me}{4} The comparison between models to identify the best model should be made in the test set.\\
		\acron[M]{me}{5} Previously annotated data should be used when testing ML models with unit tests.\\
		\acron[M]{me}{6} The performance and the time required to train a model should be taken into account when comparing models.\\
		\acron[M]{me}{7} The membership of the testing data to the training data should be tested.\\
		\acron[M]{me}{8} When cross-validation is used for testing, then the hold-out set should not be used.\\
		
		\midrule
		\multicolumn{1}{c}{\textbf{Model Deployment (md)}}\\
		\midrule	
		\acron[M]{md}{1} A deployed model should be the one that has the best hyper-parameters, but it should be re- trained with the entire dataset .\\
		\acron[M]{md}{2} When deploying a model, the entire pipeline should be exported instead of exporting only the model.\\
		
		\midrule
		\multicolumn{1}{c}{\textbf{Model Monitoring (mm)}}\\
		\midrule	
		\acron[M]{mm}{1}  After deployment, the new data that will serve as input for the model should be constantly monitored to detect any deviation from the original data.\\
		\acron[M]{mm}{2} When monitoring the data distribution, it deviates from the original one used for training and tuning models, then the model should be retrained in order to avoid degradation.\\
		
		\midrule
		\multicolumn{1}{c}{\textbf{Model Implementation (mi)}}\\
		\midrule	
		\acron[M]{mi}{1}  For the data cleaning procedure stage, routines should be used to avoid implementing everything from scratch.\\
		\acron[M]{mi}{2} Across the ML stages, pipelines should be used to automate processes and save time in complex tasks.\\
		\acron[M]{mi}{3}  In order to enable reproducibility in data pre-processing, pipelines should be used and exported.\\
		\acron[M]{mi}{4} For each trained model, a separate file should be used in order to keep track of all the possible experiments \\
		\acron[M]{mi}{5} The (hyper-)parameters used in the training process should be documented.\\
		\acron[M]{mi}{6} Once a model is deployed and a petition of data deletion is made, the data should be deleted across the entire pipeline. \\
		\acron[M]{mi}{7}  When dealing with large datasets or large files, aspects such as parallel executions, GPU us- age, and input/output efficiency should be taken into account. \\
		\acron[M]{mi}{8}  In order to optimize, parallel execution should be used if it supported by the algorithms.\\
		\acron[M]{mi}{9}  It should be verified if both, model and dataset, fit in memory.\\
		\acron[M]{mi}{10}  When dealing with large corpus, in NLP-related tasks, sparse structures should be used to improve the implementation performance.\\
		\acron[M]{mi}{11}  When dealing with large data, resource-aware implementations should be used.\\	
		
		\bottomrule
	\end{longtable}
\end{small}


==> table_practices_md_mm.tex <==
\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Model Deployment. Including the extra considerations, where  P - Phase category related  notes,  C - additional clarifications } \label{tab:pr_md} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline 
		\endlastfoot
		%\multicolumn{2}{c}{\emph{Model Deployment (md)}}\\
		%\midrule	
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*} \end{tabular}
	 	}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**} \end{tabular} } \\
		\midrule
		\acron[M]{md}{1} &A deployed model should be the one that has the best hyper-parameters, but it should be re-trained with the entire dataset. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{md}{2} & When deploying a model, the entire pipeline should be exported instead of exporting only the model. &4&-\\
	
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\end{small}


==> table_practices_me.tex <==

\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 

		
		\caption{Validated practices in the Model Evaluation stage.Including the extra considerations, where  P - Phase category related  notes, C - additional clarifications} \label{tab:pr_me} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
		%\hline
		\endlastfoot
	%	\multicolumn{1}{c}{\textbf{Model Evaluation (me)}}\\
	%	\midrule
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*} \end{tabular}
	 	}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**}  \end{tabular} } \\
		\midrule
		\acron[M]{me}{1} &Use adversarial inputs for testing a model in order to ensure robustness. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{2}& After the best hyper-parameters are found, the model with those ``optimum" hyper-parameters should be tested in the set built for testing. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{3} &If a superset vocabulary was built for an NLP task, then the model bias should be checked. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{4} &The comparison between models to identify the best model should be made in the test set. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{5} &Previously annotated data should be used when testing ML models with unit tests. &3&C\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{6} &The performance and the time required to train a model should be taken into account when comparing models. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{7}& The membership of the testing data to the training data should be tested. &3&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{me}{8}& When cross-validation is used for testing, then the hold-out set should not be used.&3&C\\
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}\\
	\end{longtable}
\end{small}


==> table_practices_mi.tex <==

\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Implementation. Including the extra considerations, where P - Phase category related  notes,  C - additional clarifications} \label{tab:pr_mi} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		

		\endlastfoot
		%\multicolumn{2}{c}{\textbf{Model Implementation (mi)}}\\
		%\midrule	
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*} \end{tabular}
	 	} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**} \end{tabular} }\\
		\midrule
		\acron[M]{i}{1} &  For the data cleaning procedure stage, routines should be used to avoid implementing everything from scratch. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{2} &Across the ML stages, pipelines should be used to automate processes and save time in complex tasks.&4&P\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{3} & In order to enable reproducibility in data pre-processing, pipelines should be used and exported. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{4} &For each trained model, a separate file should be used in order to keep track of all the possible experiments. &4&C\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{5} &The (hyper-)parameters used in the training process should be documented.&4&C\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{6} &Once a model is deployed and a petition of data deletion is made, the data should be deleted across the entire pipeline. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{7}  &When dealing with large datasets or large files, aspects such as parallel executions, GPU usage, and input/output efficiency should be taken into account. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{8} & In order to optimize, parallel execution should be used if it supported by the algorithms. &4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{9} & It should be verified if both, model and dataset, fit in memory.&4&C\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{10}  &When dealing with large corpus, in NLP-related tasks, sparse structures should be used to improve the implementation performance. &3&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{i}{11} & When dealing with large data, resource-aware implementations should be used. &3&-\\	
		
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\end{small}


==> table_practices_mm.tex <==
\begin{small}
	\setlength{\tabcolsep}{2pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
		
		\caption{Validated practices for Model Monitoring.  Including the extra considerations, where  P - Phase category related  notes,  C - additional clarifications} \label{tab:pr_mm} \\
		
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		
	%	\hline 
		\endlastfoot
	%	\multicolumn{2}{c}{\emph{Model Monitoring (mm)}}\\
		%\midrule	
		\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
				\textbf{Validated*} \end{tabular}
		} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
			\textbf{Extra**} \end{tabular} }\\
		\midrule
		\acron[M]{mm}{1}  & After deployment, the new data that will serve as input for the model should be constantly monitored to detect any deviation from the original data. &4&-\\  \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mm}{2} & When monitoring the data distribution, if it deviates from the original one used for training and tuning models, then the model should be retrained in order to avoid degradation. &4&-\\
		
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\end{small}


==> table_practices_mt.tex <==


\begin{small}
	\setlength{\tabcolsep}{3pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 
				
		\caption{Validated practices for Model Training - Learning  subcategory. Including the extra considerations, where  P - Phase category related  notes,  C - additional clarifications} \label{tab:pr_mt1} \\
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		

		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Model Training (mt)}}\\
		%\midrule
	 	\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 			\textbf{Validated*}  \end{tabular}
	 	} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
	 		\textbf{Extra**}  \end{tabular} } \\
		\midrule
		\acron[M]{mt}{1} & If the objective is to build specialized models, then a specific model for each category in a categorical feature should be trained.&4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{2} & If the dataset that is going to be used has multiple features in different scale systems, then, invariant-algorithms like tree based algorithms should be used.&4&C, P\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{3} & When training prediction models with time series data, then, sliding windows should be used.&4&-\\ \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{4} & Test data should not be included in the training data in order to have a fair metric. &4&P\\		 \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{5}  & As many data as possible should be used when training a model. &4&C\\		\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{6} & When training a NN, dropout layer(s) should be used to avoid overfitting. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{7}  & If symmetry is needed to be avoided, in a NN, their components should be initialized with different values. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{8} & Neural Networks weights should be initialized randomly to avoid symmetry. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{9} & When training a NN, Early Stopping should be used.&4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{10} & If images are being used for NN training, it is preferable a convolutional layer than a fully connected one. &4&C, P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{11} & If a neural network stagnates with non-optimal results, then the learning rate should be decreased. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{12} & If there is not enough data when training a deep NN from scratch, transfer learning with fine tuning should be tried. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{13}&  If a deep NN does not converge in an specific number of iterations, then increasing this number should be tried. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{14}& When having a large dataset that does not fit in memory, multiples models could be first trained on random data samples, and then an ensemble with those models could be created to get a more accurate model than a base learner with fewer data. &4&C, P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{15} &A model should be retrained with an online approximation if the model needs to dynamically adapt to new patterns from the data. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{16}& If dependencies between features exist, it is suggested to used GBDT instead of a Random Forest. &3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{17} &The number of parameters of a deep NN should be proportional to the number of instances needed for training a deep NN. &3&-\\	 \cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{18} &If there is a large data variance, the number of layers in a NN must be increased. &3&P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{19} &A NN should be trained with different initialized weights several times, in order to first get an average of the results and its variance and then to get a more specific judgment of the overall performance. &3&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{20} &If a NN does not converge, then the learning rate should be reduced by a half or one third. &3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{21} &When a NN does not converge, the size of the mini-batches should be increased.&3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{22} &For faster convergence of Multi Layer Perceptrons, SGD should be used. &3&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{23}& If robustness is required in an \ac{ML} model, then, Adversarial Machine learning should be used. &3&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{24} &If the time-performance of a model is being affected due to a large time series data, then the data could be sub-sampled. &3&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{25} &When sub-sampling time-series data, it should be checked that unwanted confounding between sampled origins and seasonality in data is not being introduced. &3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{26}& Before combining models, the correlation of models' prediction should be measured. &3\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{27} &Only independent models should be combined in an ensemble.&3&C, P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{28}& When training a model with mixed type features, which includes time series features, separate models for each part of the representation should be built, and then the different models should be combined in an ensemble. &3&P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{29}& When using clustering, the model should be re-trained with new data to build more clusters and increase its efficiency. &3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{30}& In order to deal with concept drift when working with data streams, models should be retrained with small a limited number of instances.&3&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{31} &A model should be retrained in offline mode, due to this method could lead to a better global approximation.&3&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{32} &In the case of online and offline re-training are not an option, then using batch/mini-batch approach should be used.&3&-\\	 \addlinespace[1pt] 
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\vspace{-10pt}
\end{small}


==> table_practices_mt2.tex <==
\begin{small}
	\setlength{\tabcolsep}{3pt}
	\begin{longtable}{M{20pt} m{225pt} m{25pt} m{25pt}} 

		\caption{Validated practices  for Model Training  - Validation  subcategory.Including the extra considerations, where  P - Phase category related  notes, C - additional clarifications } \label{tab:pr_mt2} \\
		%\hline \multicolumn{1}{c}{\textbf{Practices}}  \\ \hline 
		\toprule
		\endfirsthead
		
		\multicolumn{4}{c}%
		{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%\hline \multicolumn{1}{|c|}{\textbf{Time (s)}} &
		%\multicolumn{1}{c|}{\textbf{Triple chosen}} &
		%\multicolumn{1}{c|}{\textbf{Other feasible triples}}
		\\ \hline 
		\endhead
		
		\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
		\endfoot
		

		\endlastfoot
		%\multicolumn{1}{c}{\textbf{Model Training (mt)}}\\
		%\midrule
		\multicolumn{1}{c}{\textbf{ID}}& \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
				\textbf{Validated*}  \end{tabular}
		} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}
			\textbf{Extra**} \end{tabular} }\\
		\midrule
		\acron[M]{mt}{33} &The optimization process should be done with a validation set. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{34} &Each model that is combined into an ensemble should be optimized independently. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{35} &In order to monitor the learning process's evolution, the model's predefined metrics should be calculated at the end of each epoch. &4&P\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{36} &When data is insufficient to split it into train, validation and test, then cross-validation should be used. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{37} &It is preferable to use cross-validation instead of a training and test data split for training and testing a model. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{38} &It is preferable to use nested cross-validation instead of a training and test split for training and testing a model. &4&-\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{39} &When training NN in order to ensure reproducibility and fair comparison, the seed used for generating random numbers in the training process should be fixed. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{40} &In order to prevent overfitting, cross-validation should be used. &4&C\\	\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{41} &In order to avoid overfitting nested cross-validation should be used. &4&C\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{42}& First tune the hyper-parameters of the  probabilistic model and then adjust the decision thresholds. &3&P\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{43}& In order to monitor the evolution of the learning process and identify issues at an early stage on it, learning curves should be plotted. &3&P\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{44}& When evaluating a model, bootstrapping or cross-validation should be tried. &3&-\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{45} &When training/validating/testing a model, the process of cross-validation should be repeated with different seeds to prevent the impact of using a fixed seed. &3&C\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{46} &If you want to lower the uncertainty of the hyper-parameter tuning process, then nested cross-validation should be used. &3&-\\\cmidrule[0.01em]{1-4} \addlinespace[1pt] 
		\acron[M]{mt}{47} &In order to avoid overfitting the performance between training and testing should be compared. &3&-\\
		\bottomrule
		\addlinespace[1pt]
		\multicolumn{3}{l}{* Number of \ac{ML} experts (out of 4) that validated each practice}\\
		\multicolumn{3}{l}{** Extra considerations}
	\end{longtable}
\end{small}


==> temporal_file.tex <==
% !TEX root = main.tex



\iffalse
relu:
https://datascience.stackexchange.com/q/23493/28175
https://datascience.stackexchange.com/q/23287/28175

--- OLD VERSION


The next six practices expose the importance to consider different techniques of feature selection and their assumptions, starting with a general background check  with \acron{fe}{6}. In particular,   \acron{fe}{6}, indicates that \practice{there is a plethora of feature selection techniques  with different assumptions and purposes; therefore, when selecting features, make sure that the most suitable one is selected}; it means that there are several feature selection techniques that a practitioner should understand before using a given one in a \ac{ML} pipeline. Please note that one of the experts gave a comment to this practice, indicating that the "practice [was] too general to be useful". However, in our taxonomy we found five more detailed practices (\acron{fe}{7} - \acron{fe}{11}).%\STEFFEN{if we this is too general and we have the more detailed ones (e.g., also fe-2), why not drop this?} \ANA{We changed the redaction in order to put it a less ``obvious" way, we think that this will help us to group by  a topic and to the reader provides a starting point}


In particular, \acron{fe}{7} expresses that \practice{when using Logistic Regression} \citep{peduzzi1996simulation}  \practice{for selecting features, select the significant ones (\eg features with a \textit{p-value} smaller than 0.05)}. Selecting only the significant variables, means selecting those variables that have a smaller \textit{p-value} than the defined for the test (\eg 0.05)). When selecting those variables, we are selecting the features that rejects the \textit{null hypothesis} of the linear regression (\ie the analyzed coefficient  is equal to zero). Note that this practice has an expert comment, which says that  "logistic regression is rarely used" for feature selection. Based on that comment we investigated more about this case and we found references discussing the usage of logistic regression for feature selection \citep[\eg][]{cheng2006logistic, bursac2008purposeful, moisey2013skeletal}.%\ANA[missing]{citations, i have not found any at the moment}\STEFFEN{Look in the economics or socialogy domain. The usage of logistic regression to model something is extremely common there and they usually use p-values to determine if something had an effect.}

\acron[M]{fe}{8} indicates that \practice{ regardless the classifier that is being used,  mutual information} \citep[\eg][]{dhal2021comprehensive, sharma2018automated} \practice{ techniques for feature selection should be considered}. This feature selection could be used regardless the algorithm, since it is not related or included in any \ac{ML}, this could be done in a previous step before training.  In this case, we got a comment from one the experts saying that the practice is  "often neglected because of lacking expertise".


The next practice, \acron{fe}{9}, stipulates that \practice{using backward and forward feature selection should also be taken into account regardless of the classifier that is being used}. In other words, in the forward selection (FFS) method, we should do an iterative process,  in which we start with no variables, and in each iteration we keep adding a feature that best improves the model performance \citep{James2013}. This process of adding a variable is done  in each iteration after a round of training and testing a model for each, not previously selected, variable, and then the feature that contributes to the best model's improvement  is selected.  This process is done until the addition of a variable does not improve the performance of the model. On the other hand, the backward selection \citep{James2013}, starts with all the features, and in each iteration, the least significant  feature is removed until no improvement is observed on removal of features.  Examples of forward feature selection are \cite{rahman2020review}, in their article evaluate different methods, including FFS for autism spectrum disorder classification,  or \cite{Tang2007}, who uses FFS for mixed data with both nominal and continuous features, and examples of backward selection (BS) are \cite{Ionescu},  which use BS for query performance selection. Note that these approaches (forward and backward selection) are costly processes since training and testing of several models is required.  

In addition,  \acron{fe}{10} indicates that \practice{for feature selection, the regularization techniques that are part of the algorithm should be considered (\eg  Lasso \citep{santosa1986linear}, Elastic Net \citep{zou2005regularization}}. For example, when using Logistic Regression or a Muli layer Perceptron \citep{haykin1994neural}, feature selection with Lasso regularization should be tried, or in case of datasets with high colinearity Elastic Net should be considered. Finally, \acron{fe}{11} indicates that  \practice{the usage of Lasso \citep{santosa1986linear}, Ridge \citep{hoerl2000}, or Glmnet \citep{Jerome2010}} for feature selection in a multiple regression model should be considered}. The rational behind this practice, relates to that these approaches take a fully multivariate view of a predictor/response relationship and avoid making high variance, binary decisions.  \ANA[missing]{citation}  

\STEFFEN{the example of fe10 is redundant to fe11}\ANA{lasso is  part of both practices, that is why we put in there}


\fi
%  it means that there are several feature selection techniques that a practitioner should understand before using a given one in a \ac{ML} pipeline

%Avoid making high variance, binary decisions like "this variable is completely in, this variable is completely out".
%Lend themselves naturally to cross-validation and other model validation techniques.

==> temporal_file_steffen.tex <==
% !TEX root = main.tex

\section{Results: what are the \ac{ML} best practices found in \ac{STE} websites?}
\label{sec:results}

This section presents the results achieved by  our open-coding procedure described in the previous section.
We present the validated best \ac{ML} practices grouped by the associated \ac{ML} pipeline stage. For each practice we provide examples and extended explanations. In addition, we report  references to existing literature that could be used by the readers to get more knowledge about how to use the practices.

We present the validated ML best practices, \ie the practices reported by practitioners in STE websites and selected as good practices by the majority of the four experts involved in our study (\ie at least three experts). %In the cases in which there was at least one  "YES, but" by the experts, we will use the following notation: \ybbt{X}{j}{k},  where $X$ defines the total number of experts that validate the practice, from those experts $j$ indicated ``YES" and $k$  indicated ``YES, but". For instance,  \ybbt{4}{3}{1}  means that $4$ authors agreed, in which 3  of them said: ``yes" (\ie $y=3$) and 1 of them (\ie $yb=1$) said: ``YES, but" (\ie the authors agreed that was a good practice, an in addition, they wanted to add extra information).  
When describing the practices, we refer to each one by using an acronym composed of the \emph{stage} id and a number  $i$ ($stage_i$); for instance,  ($mr_1$) means that it is the 1$^{st}$ practice in the model requirements (\emph{mr}) stage.


\subsection{Model Requirements (mr)}

\STEFFEN{Maybe start these sections with a one-sentence description of the stage and then given the empirical data about the practices?}
\STEFFEN{Maybe add a table with all practices and identifiers and refer to this table in these sections? currently, it is difficult to just read the catalog of practices, i.e., our main result.}
Four \ac{ML} best practices were identified for this stage. Three of these practices were accepted by the four experts as best practices (\acron{mr}{1} - \acron{mr}{3}), and the  fourth \ac{ML} practice (\acron{mr}{4})  was accepted by three \ac{ML} experts. Note that, in general, in this stage, designers decide  the functionalities that should be included in the ML system, their usefulness for new or existing product,  and  the most appropriate type of ML model for the expected system features.  

The first practice (\acron{mr}{1}) relates to metrics selection, and it states that  \practice{the goal of the model that is going to be trained should be considered when selecting  the most appropriate metrics for assessing the model performance/accuracy}. For instance, if the goal/requirement is to build a more precise model  than one that retrieves all the relevant instances (\ie all the instances that are important for the task),
%\MARIO{Ana, this should be a self explained document. What do you mean with the relevant instances?} % I wil explaint it, however, for me this is a basic concept that somone that is reading about BP in machine learning has to dominate
then a metric that focuses on \STEFFEN{Here you already use precision in the sense of the metric, immediately afterwards, you use the upper-case writing for the metric. There is a good chance that readers will be confused by this.}precision is needed, like \textit{Precision} or \textit{F-score} with a $ \beta $ coefficient that favors precision\ANA[missing]{citation}.  For example, for the task of classifying X-rays as images with malignant tumors,  some of the decisions to take into account would be (i)  would it be better to retrieve with the model all the  images with malignant tumors (\ie relevant images), regardless some of the retrieval images would be  false positive (\ie images classified as relevant ones, but in reality they do not have malignant tumors)? ,  (ii) or maybe it would be better to retrieve some of the relevant images with a high certainty, decreasing the false positive images, but also missing to retrieve some images  with malignant tumors (\ie relevant images)?; (iii) or maybe it desirable to have a model that balances the  two aforementioned cases?  In the first case, the model would be focused on \STEFFEN{style for metrics above was upper case with textit, this should be consistent}recall (\ie retrieving  as many relevant images as possible); in the second case the classification model would be focused on \STEFFEN{style}precision; and in the third case, the model would be focused on balancing the two  aforementioned metrics\STEFFEN{possibly add: i.e., F-score}. 

Aligned with the \acron{mr}{1} practice the second practice (\acron{mr}{2}) suggests that \practice{it is important to identify the needs/requirements of model retraining, \eg whether it should be online, periodically, or in batch}; for instance, if you need to update a model each time that a user interacts with the model or when the data is being updated, an online approach is \STEFFEN{more than what? I suggest to drop more}more  suitable for this case.  The third practice (\acron{mr}{3}) relates to a model execution:  \practice{if a ML model  is published as a cloud service,  specifically, when a classification/prediction task uses ML cloud-based services, it is important to define the use case and the model requirements in order to identify how frequently the service should be invoked}. %; thus, having a cloud model which classifies social network posts into it respective sentiment. 
%For instance, if a cloud model is constantly classifying posts from social networks, then it should be called more frequently than a model that classifies a group of posts at the end of each day. 
This is in particular important for selecting the model and for provisioning the infrastructure required to execute the model, for instance, if a cloud model is expected to constantly classify posts from social networks, then it requires a more performant model and infrastructure than a use case in which the  model  classifies a group of posts at the end of each day. 



%also relates to a task that could be done repetitively, calling the model (\ie using the model capacity to predict/classify instances).(\textbf{mr3}) Specifically, when the action of classifying/predicting uses external services such us Cloud service, it is important to identify the use case and the model requirements in order to identify the frequency service call \ybbt{4}{4}{0}; thus, having a cloud model which classify social network posts into it respective sentiment. Thus, if a cloud model is classifying constantly post from social networks, then, it should be called more frequently than a model that classifies a group of posts at the end of each day. 


The fourth practice (\acron{mr}{4})  indicates that \practice{when using \emph{probabilistic forecasting} in a decision system, it is necessary to decouple the probabilistic model optimization from the probability threshold selection}. %\ybbt{3}{2}{1}}.  
In other words, the model hyper-parameters should be trained first, and then, the decision threshold should be adjusted. Adjusting this threshold will trade-off  between \textit{True Positives} (\textit{TP}) (\ie  number of positive instances correctly classified) and \textit{False Negatives} (\textit{FN}) (\ie  number of negative instances incorrectly classified), as well as  \textit{False Positives} (\textit{FP}) (\ie number of positive instances incorrectly classified)  and \textit{True Negatives} (\textit{TN}) (\ie number of negative instances correctly classified).  In other words adjusting the threshold could cause that some of the instances classified as TP could be classified as FN and the same with FP and TN. To illustrate this, imagine that a logistic regression model is used for identifying vulnerable or not vulnerable code snippets.  As \acron{mr}{4} indicates, in first instance the logistic regression should be trained in order to find the optimum hyper-parameters (\eg solver, penalty and $C$), then,  the decision threshold should be adjusted. Now, let's assume that we have a  binary decision system (\eg fix or not a potentially vulnerable code) and  that the vulnerabilities that are being detected have a low score in the  \textit{CVSS} \footnote{The common vulnerability Scoring system (https://nvd.nist.gov/vuln-metrics/cvss)} rating.  Then, if some vulnerable code snippets are being classified as not vulnerable (FN), thus, those snippets will not be fixed. It will be less crucial  that if those vulnerabilities had a critical score in the same ranking. In consequence, in this case, adjusting the threshold in order to trade off between TP for FN and FP for TN  %\MARIO{what do you mean wit trade off between x for y? where did you get that grammatical structure from?} \ANA[missing]{ from Books}
will be useful depending on the cost of classifying  an instance incorrectly.  On the other hand, we could also be in a scenario in which we have a binary target (\eg vulnerable or not) but multiple decision thresholds associated to it  (\eg not fixing it, fixing it in one hour, one day, or in a week). In this second case, each threshold, associated to a fixing period, has to be also adjusted after optimizing the  logistic regression.  It is important to note, that three authors validated the \acron{mr}{4} practice, however, one expert answered with "YES, but". The clarification given by that experts is that ``I think this GP belongs to the training category".  We decided that this practice still belonged to this stage, since it is  the decision process on how the model will be trained, it is not the training process itself.\STEFFEN{I tend to agree with the expert here. But this is really borderline. The question is: is it worth it that we argue against the expert here or should we just move it to avoid a reviewer comment like "why did you use experts when you overrule them anyways?"} 

%\MARIO{We have to explain why did we include mr4 in mr instead of training. } 


\subsection{Data Collection (dc)}
This second stage encompasses  all the processes of looking for and integrating available datasets and also collecting them. Datasets can be created from scratch, or  existing datasets  can be used to train models in a transfer learning fashion. Both scenarios are widely used when creating ML systems.  In this stage, seven validated practices were identified, three of them were validated by all of the experts (\acron{dc}{1}-\acron{dc}{3}) and the remaining four (\acron{dc}{4} - \acron{dc}{7}) by three of the experts.  It is worth noting that the identified practices relate to some characteristics that the collected data has to meet during/after this process.\STEFFEN{Why is this worth noting? seems obvious to me, what else should it be about?}

The first practice (\acron{dc}{1})  refers to  data distribution, indicating that \practice{the distribution of the training data (\eg data used to train the \ac{ML} model) should reflect the real distribution (\ie original distribution of the population from which the data was extracted)}.  This is because machine learning models try to approximate the \textit{real-world distribution} based on the training data. If a completely different distribution is passed as input for training, then the model is going to approximate to a distribution that do not exists in real life, and it is going to have a bad performance \ANA[missing]{citation}. In addition,  (\acron{dc}{2}) suggests that \practice{if a model is expected to detect ``something'' in an image, then representative examples of that ``something'' should be present in the training and testing data}.  For example, let us assume that a ML model is expected to recognize a component  --- of  a mobile interface --- such as a button or a text area in UI screenshots; then, according to the \acron{dc}{2} practice the data used for training and testing should have  images in which the component is exhibited. It is important to clarify, that \acron{dc}{2} also implies that the ``context'' of the detected object  is relevant (\eg background). For instance, if the model  now has to identify buttons in dark backgrounds, then  the training data should also include those types of images. Although this practice is reported by STE practitioners in the specific domain of images, it can be generalized to other artifacts (\eg text).


The third data collection practice (\acron{dc}{3}) indicates that \practice{when measuring  a dataset size it should not be done  only by referring to storage space (Mb, Gb) but also in terms of rows and columns}. Measuring  the size of a data set only in terms of storage space, is often misleading, making the dataset seem more gigantic than it is. %\MARIO{Why  is it misleading?}. Mario, the sentence next to the missleading explains why
\STEFFEN{I think the issue is still open, i.e., I do not see an explanation why size is not a good proxy}
In addition, in some cases, having the size of the matrix (\ie rows and columns) that is going to be used by the \ac{ML} model  could help to compute the model's complexity or  estimate the execution time in advance. \ANA[missing]{references}


The second group of data collection practices (\acron{dc}{4} - \acron{dc}{5}) is mainly about negative samples (\ie the instances of the  class that is not the target of a binary classifier),  and in particular, they are about images belonging to a negative class. The fourth data collection practice (\acron{dc}{4}) indicates that \practice{if it is required to augment the number of instances  in the negative class, pre-existing  datasets could be used  for including more instances in the dataset}. For instance, if a model is classifying  whether a UI has buttons or not, then you could augment your dataset with instances from the RICO dataset (\cite{DEKA_2017}) as a generic dataset that contains images with mobile interfaces to find samples of a negative class (\eg views without buttons).  The fifth practice  (\acron{dc}{5}) indicates that \practice{the images that are going to be used as instances of the negative class should have some common characteristics with the positive ones}. This means, that the negative samples should ``look similar'' to the positive ones; in this way, the model will learn special features that will help to differentiate a particular object to similar ones. For instance, when classifying images that contain buttons, a good idea will be to include in the negative sample images with components that look similar to buttons (\eg cards).  

The following two practices relate specifically to object detection tasks. \acron[M]{dc}{6}  suggests that \practice{the minimum size of the object that is going to be detected should be present in the data that is going to be used for training the model}; and \acron{dc}{7} indicates that \practice{the object regions of interest (ROI)  (\ie region in which the object to be detected is present)  should have a similar aspect ratio in all the positive images}. These two practices could be exemplified as follows. Imagine  that the classification button problem now includes the detecting of the exact position of buttons in  images of mobile apps. Following \emph{\acron[M]{dc}{6}},  if the smaller button that is going to be detected is 10dp, then images with buttons of that size should de present in the training data. Following \acron{dc}{7},  means that it  is important to ensure that the aspect ratio of the region in which the button is present is maintained in all the positive images.  These two practices are relevant since \acron{dc}{6} guarantees that the minimum size of an important feature (\eg angle, size, curve) is being observed by the detection model, therefore could be learned and  \acron{dc}{7} indicates which aspect ratio the important features (\ie features that could help to detect an object) are going to have. \ANA[missing]{citation}

% \MARIO{Ana, why? We need to explain why dc6 and dc7 should be followed, and include refs}

\STEFFEN{Finished until here}
\subsection{ Data Cleaning (dcl)}

This is the second stage in which the most practices were identified (\ie 33 practices). In general, this stage involves removing inaccurate or noisy records from a dataset (\cite{amershi2019software}).  %, with 33  best validated practices 20 practices validated by all exerts and 13 validated by three of them.  
In this case,  we will present the practices aggregated by three  subcategories: Exploratory data analysis (EDA), Wrangling, and Data.% inside each of these groups we will present the previous used division (\ie practices validated by all the experts and practices validated by three of them). We do this division in order to facilitate the reading of the 33 practices. 


\textbf{EDA.} We consider it as the first subcategory of data wrangling, since a possible first step to modify/pre-process/wrangling data is to understand them and their characteristics (\eg trends, nature, format). This understanding could be done through a exploratory data analysis.  Regarding this procedure, we identified a total of seven validated practices; six practices were validated by all the experts (\acron{dcl}{1} - \acron{dcl}{6}) and one  was validated by three of them (\acron{dcl}{7}). 


The first identified practice (\acron{dcl}{1}), indicates that \practice{for each possible attribute/column in a dataset, we should identify its type  (\eg numeric, categorical, time data) before applying any pre-processing technique}. This practice is relevant since some pre-processing techniques are not valid for all the data types \ANA[missing]{group of citations}, for example if a categorical variable is represented  with number it does not mean that it could be normalized. In addition, some \ac{ML} models   do not receive all kind of data as input. 
%\MARIO{Please clarify that some pre-processing techniques are valid with some types of data.... give examples and references}

The second practice, \acron{dcl}{2},  indicates that \practice{it  should be  determined what variables are dependent and what ones  are independent}. In this way, it could be determined which attributes could be used as features/measured variables and what ones  could be  target(s)/response variable.%\MARIO{Why?} 
It is worth mentioning that two "YES, but" observations were given by the experts. The first one says that  ``its usually limited [the determination of dependent and independent] to linearity measures - which is not always appropriate", showing us the importance of understanding what does it mean to be dependent. In addition,  the second comment indicates that the practice depends on the problem and the selected algorithm; the second expert also leaved an open question about whether the analysis is feasible when having a dataset  with thousands  of variables.
\MARIO{So, what can we do in this case?} \ANA{i do not know, i have to search more} 

The following two practices deal with the identification of trends in data.  \acron[M]{dcl}{3} specifies that \practice{when analyzing time series/temporal data, possible temporal trends should be identified (\eg every Monday, January, every two weeks)}. For example, a dataset of fixed vulnerabilities is being analyzed,  when analyzing it, fixing a huge amount of vulnerabilities every last Friday of the month is detected as a trend. These kind of insights could be useful for the model as a new feature (\eg each Monday developer 1 add more lines of code than any other developer)%\MARIO{So...what? what can we do with those trends? Why is is important to identify the trends?} 
Moreover,  \acron{dcl}{4} indicates that \practice{weird trends (\ie trends that need to cross reference the data against  an external source that maps time events) should also be identified}.  For instance,  let us assume the periods where least vulnerabilities are fixed are Christmas and new years eve, then this could be a new feature which indicates a cause of why in some periods the issues take longer to be solved.  %\MARIO{?? Please finish the example}. 


The following two practices are about identifying missing data and possible errors in it.  In particular,  \acron{dcl}{5} expresses that \practice{it is needed to identify missing values and their nature before doing any pre-processing}. In particular, missing values in a variable/feature could be valuable;  thus, removing it before analyzing and understanding them could cause data losses.  Moreover,  \acron{dcl}{6}  indicates that \practice{before applying any pre-processing technique, potential errors in data should be identified}. For example, if at some point of time data records the format changed, {\eg from \textit{MM/DD/YYYY} to \textit{DD/MM/YYYY}) it should be noticed at this stage; otherwise, the month and day could de exchanged without any notice. %\MARIO{why?}
	
	
	
The last, but not least, data cleaning practice (\acron{dcl}{7}) in the \emph{EDA}  subcategory was validated by three authors.  This practice is about geographical  data (\ie data that is associated to a particular geographical space), and it indicates that   \practice{ if correlation between existing features and instances of geographical  data  are needed, then, geographical  data  should be clustered}.  In other words, when clustering geographical data similar data points are grouped which facilitates the identification of relations between a targeted class and the geographical features.
%\MARIO{why?}% no encontré ningún ejemplo para usar software acá, dejar el caso de datos geograficos  % practice: cluster geo located data in order to find correlations between a target class and the existing features and instances


\textbf{DATA.} %\MARIO{Why did we call this category DATA?} 
In this  subcategory, we present practices that deals with splitting the dataset and a practice related to when to measure (\ie determining the size of the dataset)%\MARIO{what do you mean with measure?} 
a dataset.  This subgroup is called Data, since we present practices related to the data and dataset themselves and not to any ore-processing or analysis. In this group, four validated practices were identified, two of these practices (\acron{dcl}{8}, \acron{dcl}{9}) were validated by four experts and the remaining ones (\acron{dcl}{10} and \acron{dcl}{11}) were validated by three \ac{ML} experts. 


On the one hand, \acron{dcl}{8} indicates that \practice{for improving model performance  with a dataset that has  a categorical feature, the data should be split by each category}.  To illustrate this, imagine that a model is needed to predict how many hours are needed to fix a bug, the input dataset has a variable that indicates the component in which the developer is working (\eg back-end and front-end). Then, following \acron{dcl}{8}, the dataset should be grouped by each component, back-end and front-end, and afterwards each model should be trained separately in order to have a model specialized to predict the amount of time needed to solve and issue per area.  %\MARIO{Why do we have to do the splitting?} 
Note that one \ac{ML} expert gave a comment to this practice:  a better way to refer to this practice could be ``model specialization". On the other hand,  \acron{dcl}{9} expresses that \practice{if in the model training stage it is needed to optimize hyper-parameters, the dataset should be split into training, validation and test sets in order to prevent overfitting and avoid biased computing  metrics}.  In this way, the model is going not going to have a biased metric neither for the selection of the hyper-parameter nor the model selection (\ie testing the final model in the test set). It is worth mentioning that an expert left a comment indicating that it would be better to refer to this practice as ``data partition". % \MARIO{Why do we need to have that data partitioning schema?} as it is mentioned in the next phrase it is to avoid overfitting and avoid biased metric :) ; however i added another sentence


The following two practices in this category also relate to the training and testing stages. In particular,   \acron{dcl}{10} relates to the training stage; it describes that \practice{in order to prevent overfitting and avoid biased metrics when optimizing  the whole dataset, it should be divided into train and test; then, the training data should be divided into folds for cross-validation}. Note that, an expert left a comment indicating that this practice should be referred as ``data partition".  As it was previously mentioned, when separating the training data from the other sets it allows to (i) avoid overfitting, since the model is not going to learn the whole dataset by ``memory" and (ii) it allows to have another set for testing the model in which a fair metric can be calculated, since the data has not been previously seen. 
%\MARIO{Ana, discuss the practice} DONE

Finally,  \acron{dcl}{11}  indicates that \practice{the size of a dataset should be only calculated after the data pre-processing}.  This is because features and records could be deleted or added in the pre-processing process, which changes the original size of the raw data. 


\textbf{Wrangling}. In this subcategory we grouped all the practices that munge/transform the raw data into another format  that will be useful when training the models. In this case 22 practices were accepted, 12 of them were validated by the four the experts, and 10 were validated by three experts. 

The first wrangling practice, \acron{dcl}{12},  expresses that \practice{if an imputation (\ie replacement of missing values) technique is used, then, the same technique should be used in the validation and testing sets}.  When imputing a dataset the same as the following transformations, it should be done at first only taking into account the training data, in this way no information of the remaining dataset is being learned; then the learned information about how to impute the missing data should be applied into the remaining set. This  execution should be done, since if the imputation is not applied to the remaining data, the training data would have different format and distribution than the other data. \ANA[missing]{citation}. Note that any kind of imputation could  introduce a biased, since the distribution is being affected. \ANA[missing]{citation}
%\MARIO{Ana, discuss the practice}


The next three practices are related to unbalanced data. Firstly,  \acron{dcl}{13} describes that \practice{when having an unbalanced dataset, balancing the data (\ie process in which an unbalanced dataset is treated to have an equal or almost equal number of samples from each class) should be done only in the training dataset}. Secondly, \acron{dcl}{14} states that \practice{when undersampling data (\ie technique to balance uneven datasets by decreasing the size of the majority class by selecting some samples and   keeping all of the data in the minority class),  the samples that are being selected should be randomly sampled}. Thirdly,  \acron{dcl}{15}  mentions that \practice{oversampling  (\ie technique to balance uneven datasets by duplicating samples from the minority class) should be done only after the whole dataset is split into train, validation and test sets}.  It is worth mentioning that an expert left a comment  indicating that this group of practices belongs more to another group of practice, ``DATA", %\MARIO{Which one?} 
and not wrangling. However, we kept them in this group since handling a imbalanced dataset involves munging it.  It is important to note, that imbalanced dataset could be a challenge since most of the \ac{ML} algorithms used for classification were designed having as bases an balanced classes (\ie equal number of instances per each class). This could lead to  poor performance models, especially for the minority class (\ie class with fewer examples); since the model has few examples of the class to learn from.  \ANA[missing]{citation} In  addition, when calculating performance metrics, this should be taken into account \ANA[missing]{citation}  is different to have a precision of 100\% when only a single practice was evaluated (1 practice classified right out of 1 possible practice) that having 300 out of 300 well classified. How the dataset should be imputed, depends on multiple factors such as which is the minority class (the main class of interest) or other class; determining the type of difference between each class. \ANA[missing]{citation}  %\MARIO{Ana, discuss the practices? what are the issues with imbalanced data? when undersample and why? when oversample and why?}

\ANA{Steffen until here we have completed a complete review :)}



==> temporal_filetwo.tex <==
% !TEX root = main.tex


\iffalse
relu:
https://datascience.stackexchange.com/q/23493/28175
https://datascience.stackexchange.com/q/23287/28175

--- OLD VERSION

% !TEX root = main.tex


The next three practices are related to unbalanced data. Firstly,  \acron{dcl}{13} describes that \practice{when having an unbalanced dataset, balancing the data (\ie process in which an unbalanced dataset is treated to have an equal or almost equal number of samples from each class) should be done only in the training dataset}. Secondly, \acron{dcl}{14} states that \practice{when undersampling data (\ie technique to balance uneven datasets by decreasing the size of the majority class by selecting some samples and   keeping all of the data in the minority class),  the samples that are being selected should be randomly sampled}. Thirdly,  \acron{dcl}{15}  mentions that \practice{oversampling  (\ie technique to balance uneven datasets by duplicating samples from the minority class) should be done only after the whole dataset is split into train, validation and test sets}

\STEFFEN{dcl-15 is a subset of dcl-13, as both lead to the same result, i.e., sampling only on the training data. This practice should be removed}. 
\ANA{I think that is not a good idea, since dcl13 is an overview of doing something only in the training data, but dcl15 is refering specially to oversample and refers to splitting data, when I was writing this practice I also thought that It was ``Obvious more after having the dcl13" but if we want that this could be useful for a rookie }

Bear in mind that an expert left a comment  indicating that this group of practices belongs more to another group of practice, ``DATA",  and not wrangling. However, we kept them in this group since handling a imbalanced dataset involves munging it.  It is to be noted that imbalanced dataset could be a challenge since most of the \ac{ML} algorithms used for classification were designed having as bases an balanced classes (\ie equal number of instances per each class). This could lead to  poor performance models, especially for the minority class (\ie class with fewer examples) due to the model has few examples of the class to learn from.  \ANA[missing]{citation} In  addition, when calculating performance metrics, this should be taken into account \ANA[missing]{citation}  is different to have a precision of 100\% when only a single practice was evaluated (1 practice classified right out of 1 possible practice) that having 300 out of 300 well classified. How the dataset should be imputed, depends on multiple factors such as which is the minority class (the main class of interest) or other class; determining the type of difference between each class. \ANA[missing]{citation}  

\fi
